Relational Proxies: Emergent Relationships as Fine-Grained Discriminators

Fine-grained categories that largely share the same set of parts cannot be discriminated based on part information alone, as they mostly differ in the way the local parts relate to the overall global structure of the object. We propose Relational Proxies, a novel approach that leverages the relational information between the global and local views of an object for encoding its semantic label. Starting with a rigorous formalization of the notion of distinguishability between fine-grained categories, we prove the necessary and sufficient conditions that a model must satisfy in order to learn the underlying decision boundaries in the fine-grained setting. We design Relational Proxies based on our theoretical findings and evaluate it on seven challenging fine-grained benchmark datasets and achieve state-of-the-art results on all of them, surpassing the performance of all existing works with a margin exceeding 4% in some cases. We also experimentally validate our theory on fine-grained distinguishability and obtain consistent results across multiple benchmarks. Implementation is available at https://github.com/abhrac/relational-proxies.

==> tex/05_discussion.tex <==
\section{Discussion}

\myparagraph{Limitations}
The process of obtaining local views in our method is somewhat of an uninformed, generic cropping methodology on the global view of the object, which may not necessarily always yield the best set of local object parts. More informed ways of detecting novel object parts from which the global view emerges can lead to obtaining at par performance but with fewer local views.

\myparagraph{Societal Impacts}
The rigorous theoretical basis of our work has a positive societal impact, which not only makes our methodology transparent and easy to analyze, but also provides a framework to study the foundations of FGVC in general.
So far, we are not aware of any negative societal impact that is specific to our methodology. However, as with all data-driven approaches, underlying biases in the datasets on which our model is trained would influence the patterns learned by it.

